SMURF: Continuous Dynamics for Motion-Deblurring Radiance Fields

Neural radiance fields (NeRF) has attracted considerable attention for their exceptional ability in synthesizing novel views with high fidelity. However, the presence of motion blur, resulting from slight camera movements during extended shutter exposures, poses a significant challenge, potentially compromising the quality of the reconstructed 3D scenes. To effectively handle this issue, we propose sequential motion understanding radiance fields (SMURF), a novel approach that models continuous camera motion and leverages the explicit volumetric representation method for robustness to motion-blurred input images. The core idea of the SMURF is continuous motion blurring kernel (CMBK), a module designed to model a continuous camera movements for processing blurry inputs. Our model is evaluated against benchmark datasets and demonstrates state-of-the-art performance both quantitatively and qualitatively.

==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Neural Radiance Fields (NeRF)}
\label{subsec:related_nerf}

The synthesis of photo-realistic novel views from images of different viewpoints has attracted considerable attention with the advancement of NeRF~\cite{mildenhall2020nerf}. In particular, NeRF uses 3D spatial coordinates and 2D viewing directions to map radiance and volume density, a process facilitated by implicit neural representation (INR). Following the success of NeRF, various sub-domains considering real-world scenarios have been explored. Many recent studies have extensively applied NeRF across various fields, including dynamic 3D scene modeling~\cite{park2021nerfies,li2021nsff,pumarola2021dnerf,tretschk2021nonrigid,park2021hypernerf,li2022neural3dvideo,lombardi2019neural,zhang2021editable,cao2023hexplane}, scene relighting~\cite{srinivasan2021nerv,bi2020neuralreflectappear,martin2021nerfinthewild,philip2021free,toschi2023relight}, and 3D reconstruction~\cite{wang2021neus,sun2021neuralrecon,wen2023bundlesdf}. Furthermore, recent studies have applied NeRF for deblurring 3D scenes~\cite{ma2022deblurnerf,lee2023dp,peng2023pdrf,wang2023bad}, assuming blurry input images from real-world conditions and aiming to produce clean images. Additionally, due to the slow rendering caused by the costly MLP layers required to evaluate each pixel's density and color, some studies~\cite{kurz2022adanerf,piala2021terminerf,neff2021donerf,chen2022tensorf,muller2022instant,yu2021plenoxels,sun2022direct} design networks for faster training and rendering. To address these challenges, various voxel-based explicit rendering methods~\cite{chen2022tensorf,muller2022instant,yu2021plenoxels,sun2022direct} have been proposed, offering competitive performance to NeRF while significantly reducing training and rendering times. We adopt an explicit representation method, TensoRF~\cite{chen2022tensorf} as the backbone, which facilitates fast training and achieves accurate and efficient novel-view rendering.

\subsection{NeRFs from Blurry Images}
\label{subsec:related_deblur_nerf}

Recently, several studies have been conducted to deblur 3D scenes and synthesize clean novel view images using blurry input images from different views. Deblur-NeRF~\cite{ma2022deblurnerf} proposes, for the first time, an implicit blurring kernel in 3D space inspired by blind deblurring methods for 2D vision~\cite{krishnan2011blind,joshi2009deblurcolorpirors,sun2015learningcnndeblur}. This blurring kernel is intentionally trained close to the pixels of the blurry image, and during rendering, a clean image is obtained without the trained kernel. DP-NeRF~\cite{lee2023dp} models a rigid kernel that assumes physical scene priors when blurry images are captured. BAD-NeRF~\cite{wang2023bad}, assuming a very short camera exposure time, designs a kernel that linearly interpolates the camera motion trajectory in using simple spline-based method. Recently, methods utilizing 3DGS have been proposed to enable faster rendering. For instance, Deblurring 3DGS~\cite{lee2024deblurring} adjusts Gaussian parameters like rotation and scaling to generate blurry images during training, and BAGS~\cite{peng2024bags} proposes a blur-agnostic kernel and a blur mask using convolutional neural networks (CNNs). However, these approaches estimate the change in camera pose jointly, not modeling the fact that light traces left by camera motion during exposure time appear continuously. Therefore, we aim to design a kernel where the elements of the blurring kernel, namely the small changes in camera pose, are estimated sequentially over time.


\subsection{Neural Ordinary Differential Equations}
\label{subsec:related_neural_ode}

Neural-ODEs~\cite{chen2018neural} are proposed to interpret neural networks within the framework of ordinary differential equations, representing the underlying dynamics inherent in hidden parameters. Neural-ODEs model a parameterized time-continuous latent state and output a unique solution of the integral of continuous dynamics, utilizing given initial values and various numerical differential equation solvers (\textit{e.g.} Euler's method~\cite{euler1845institutionum}, Runge-Kutta method~\cite{kutta1901beitrag}, Dormand-Prince-Shampine method~\cite{dormand1980family}). They are extensively used to continuously connect the latent space embedded in videos~\cite{kanaa2021simple,park2021vid,fernandes2019predicting,hofherr2023neural} or model the continuous dynamics of irregularly sampled time-series data~\cite{rubanova2019latent}. Inspired by the fact that camera motion is continuous, we exploit Neural-ODEs to create a precise blurring kernel that models the hidden continuous dynamics inherent in camera motion.

==> sec/6_limitation.tex <==
\section{Limitations and Future Work}

By adopting TensoRF~\cite{chen2022tensorf}, a 3D tensor factorization-based method, as our backbone, we ensure high quantitative performance, superior perceptual quality, and faster training. However, with the advent of 3D Gaussian Splatting~\cite{kerbl20233d}, which allows for GPU-based rasterization instead of ray tracing-based methods, backbones that facilitate more faster training and rendering become available. Although our backbone shows slower training and rendering speed compared to 3D Gaussian Splatting, applying the main idea of CMBK, \textit{continuous dynamics}, to a rasterization-based method is expected to result in faster training and rendering with superior perceptual quality. Furthermore, by demonstrating the applicability of \textit{continuous dynamics} to the 3D scene deblurring, we anticipate the possibility of designing models that cover not only camera motion blur but also object motion blur, which is caused by the movement of objects within the scene.
